Pots of Gold at the End of the Rainbow: What is Success for Open Source Contributors?

Success in Open Source Software (OSS) is often perceived as an exclusively code-centric endeavor. This perception can exclude a variety of individuals with a diverse set of skills and backgrounds, in turn helping create the current diversity & inclusion imbalance in OSS. Because people's perspectives of success affect their personal, professional, and life choices, to be able to support a diverse class of individuals, we must first understand what OSS contributors consider successful. Thus far, research has used a uni-dimensional, code-centric lens to define success. In this paper, we challenge this status-quo and reveal the multi-faceted definition of success among OSS contributors. We do so through interviews with 27 OSS contributors who are recognized as successful in their communities, and a follow-up open survey with 193 OSS contributors. Our study provides nuanced definitions of success perceptions in OSS, which might help devise strategies to attract and retain a diverse set of contributors, helping them attain their "pots of gold at the end of the rainbow".

==> Tables/codes.by_role.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htb]
\centering
\caption{Quadrants and Regions cited by the Interview's Participants who play roles as coders and non-coders}
\label{tab:codes_by_role}
\footnotesize
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Quadrant}                     & \multirow{2}{*}{Region} & \multicolumn{2}{c|}{Participants ID}            \\ \cline{3-4} 
 &             & Coders (12)               & Non-Coders (15)                \\ \hline
\multirow{2}{*}{Intra-Personal x Affect}      & Satisfaction            & P5, P21                    & P1, P10, P16, P26      \\ \cline{2-4} 
 & Security    & P19, P24             &                           \\ \hline
\multirow{2}{*}{Intra-Personal x Achievement} & Self-Development        & P7, P18, P19, P20, P21, P24 & P12, P16          \\ \cline{2-4} 
 & Creativity  &                      & P10                       \\ \hline
\multirow{3}{*}{Inter-Personal x Affect}      & Perceived Contribution  & P5, P6, P18, P21, P25       & P22, P9, P11, P17 \\ \cline{2-4} 
 & Cooperation & P2, P5, P7, P20, P21 & P3, P4, P8, P13, P15, P17 \\ \cline{2-4} 
 & Recognition & P23, P25, P27             & P1, P9, P13, P22          \\ \hline
\multirow{3}{*}{Inter-Personal x Achievement} & Factual Contribution    & P2, P6, P18, P19, P20, P21  & P12, P14          \\ \cline{2-4} 
 & Advancement & P20, P21, P23, P24, P27   & P1, P10, P16, P22         \\ \cline{2-4} 
 & Performance &                      & P4                        \\ \hline
\end{tabular}
\end{table*}

==> Tables/codes_new.tex <==
\begin{table*}[htb]
\centering
%\scriptsize
\caption{Success meanings from the interviews and the survey classified per Dries et al.'s  model \cite{dries2008career}}
\label{tab:codes}
\footnotesize
\resizebox{0.95\textwidth}{!}{%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{tabular}{c|c|c|c|l|r|r}
\hline
\rowcolor[HTML]{C0C0C0} 
\begin{tabular}[c]{@{}l@{}} Affect $\times$\\ Achievement\end{tabular} &
  \begin{tabular}[c]{@{}l@{}} Interpersonal $\times$ \\ Intrapersonal\end{tabular} &
  Quadrants &
  Region &
  Participants' IDs (Interviews) &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}\# Interviews\\ total: 27\end{tabular}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}\# Survey\\ total: 193\end{tabular}} \\ \hline\hline
 &
   &
   &
  Cooperation &
  P2, P3, P4, P5, P7, P8, P13, P15, P17, P20, P21 &
  11 &
  19 (8\%) \\ \cline{4-7} 
 &
   &
   &
  Perceived Contribution &
  P5, P6, P9, P11, P17, P18, P21, P22, P25 &
  9 &
  57 (30\%) \\ \cline{4-7} 
 &
   &
   &
  Recognition &
  P1, P9, P13, P22, P23, P25, P27 &
  7 &
  29 (12\%) \\ \cline{4-7} 
\multirow{-4}{*}{Affect} &
   &
  \multirow{-4}{*}{Quad1} &
  \multicolumn{2}{r|}{\cellcolor[HTML]{EFEFEF}Participants who mentioned at least one Region from Q1} &
  \cellcolor[HTML]{EFEFEF}20 &
  \cellcolor[HTML]{EFEFEF}93 (48\%) \\ \cline{1-1} \cline{3-7} 
 &
   &
   &
  Advancement &
  P1, P10, P12, P16, P20, P21, P22, P23, P24, P27 &
  9 &
  8 (4\%) \\ \cline{4-7} 
 &
   &
   &
  Performance &
  P4 &
  1 &
  0 (0\%) \\ \cline{4-7} 
 &
   &
   &
  Factual Contribution &
  P2, P6, P12, P14, P18, P19, P20, P21 &
  8 &
  74 (38\%) \\ \cline{4-7} 
 &
   &
  \multirow{-4}{*}{Quad2} &
  \multicolumn{2}{r|}{\cellcolor[HTML]{EFEFEF}Participants who mentioned at least one Region from Q2} &
  \cellcolor[HTML]{EFEFEF}15 &
  \cellcolor[HTML]{EFEFEF}81 (42\%) \\ \cline{3-7} 
\multirow{-5}{*}{Achievement} &
  \multirow{-9}{*}{Interpersonal} &
  \multicolumn{3}{r|}{\cellcolor[HTML]{E6E5E5}Participants who mentioned at least one Region from Interpersonal} &
  \cellcolor[HTML]{E6E5E5}26 &
  \cellcolor[HTML]{E6E5E5}162 (84\%) \\ \hline
 &
   &
   &
  Self-Development &
  P7, P16, P18, P19, P20, P21, P24 &
  7 &
  19 (8\%) \\ \cline{4-7} 
 &
   &
   &
  Creativity &
  P10 &
  1 &
  2 (1\%) \\ \cline{4-7} 
\multirow{-3}{*}{Achievement} &
   &
  \multirow{-3}{*}{Quad3} &
  \multicolumn{2}{r|}{\cellcolor[HTML]{EFEFEF}Participants who mentioned at least one Region from Q3} &
  \cellcolor[HTML]{EFEFEF}8 &
  \cellcolor[HTML]{EFEFEF}21 (11\%) \\ \cline{1-1} \cline{3-7} 
 &
   &
   &
  Satisfaction &
  P1, P5, P10, P16, P21, P26 &
  6 &
  13 (5\%) \\ \cline{4-7} 
 &
   &
   &
  Security &
  P19, P24 &
  2 &
  17 (7\%) \\ \cline{4-7} 
 &
   &
  \multirow{-3}{*}{Quad4} &
  \multicolumn{2}{r|}{\cellcolor[HTML]{EFEFEF}Participants who mentioned at least one Region from Q4} &
  \cellcolor[HTML]{EFEFEF}8 &
  \cellcolor[HTML]{EFEFEF}30 (16\%) \\ \cline{3-7} 
\multirow{-4}{*}{Affect} &
  \multirow{-7}{*}{Intrapersonal} &
  \multicolumn{3}{r|}{\cellcolor[HTML]{E6E5E5}Participants who mentioned at least one Region from Intrapersonal} &
  \cellcolor[HTML]{E6E5E5}11 &
  \cellcolor[HTML]{E6E5E5}49 (25\%) \\ \hline
\rowcolor[HTML]{E6E5E5} 
\multicolumn{5}{r|}{\cellcolor[HTML]{E6E5E5}Participants who mentioned at least one Region from Affect} &
  25 &
  49 (25\%) \\ \hline
\rowcolor[HTML]{E6E5E5} 
\multicolumn{5}{r|}{\cellcolor[HTML]{E6E5E5}Participants who mentioned at least one Region from Achievement} &
  17 &
  95 (49\%) \\ \hline
\end{tabular}
}

\resizebox{0.80\textwidth}{!}{%
\tiny
\begin{tabular}{r}
\textbf{Quad1}: Interpersonal x Affect; \textbf{Quad2}: Interpersonal x Achievement; \textbf{Quad3}: Intrapersonal x Achievement; \textbf{Quad4}: Intrapersonal x Affect\\
The total per quadrant is not the sum of the regions since the participants often provided an answer that was categorized into \textbf{more than one region}.
\end{tabular}
}


\end{table*}

==> Tables/codes_survey.tex <==
\begin{table*}[htb]
\centering
\caption{Success meanings from the survey classified per Dries et al.'s  model \cite{dries2008career} and per type of contribution, gender and the financial relation with OSS}
\label{tab:codes_survey}

\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{l|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
\hline
  \multicolumn{1}{c}{\multirow{3}{*}{}} &
%  \multirow{3}{*}{\textbf{Region}} &
  &
  \multicolumn{4}{c|}{\textbf{Type of Contribution}} &
  \multicolumn{6}{c|}{\textbf{Gender}} &
  \multicolumn{6}{c|}{\textbf{Employment in OSS}}&
  \multicolumn{2}{c}{}  \\ 
  \cline{3-18} 
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c|}{\textbf{Region}} &
  \multicolumn{2}{c|}{Coders} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Coders\end{tabular}} &
  \multicolumn{2}{c|}{Men} &
  \multicolumn{2}{c|}{Women} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Binary\end{tabular}} &
  \multicolumn{2}{c|}{Paid} &
  \multicolumn{2}{c|}{Unpaid} &
  \multicolumn{2}{c|}{\begin{tabular}[c|]{@{}c@{}}Partially\\Paid\end{tabular}} 
  &
  \multicolumn{2}{c}{\textbf{Total} }\\ \cline{3-20} 
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{}&
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% \\ \hline\hline

\multirow{3}{*}{Quad1} &

Cooperation &
  10 &
  6.1\% &
  5 &
  16.7\% &
  12 &
  7.4\% &
  0 &
  0.0\% &
  2 &
  100.0\% &
  5 &
  13.9\% &
  10 &
  7.3\% &
  0 &
  0.0\% 
    &
  19&
  8.0\%
  \\ \cline{2-20} 

 &

  Perceived Contr. &
  51 &
  26.4\% &
  6 &
  20.0\% &
  52 &
  31.9\% &
  3 &
  18.8\% &
  0 &
  0.0\% &
  11 &
  30.6\% &
  42 &
  30.7\% &
  3 &
  18.8\% 
    &
  57&
  29.5\%
  \\ \cline{2-20} 

 &
  
  Recognition &
  25 &
  15.3\% &
  4 &
  13.3\% &
  24 &
  14.6\% &
  4 &
  25.0\% &
  0 &
  0.0\% &
  5 &
  13.9\% &
  21 &
  15.3\% &
  3 &
  18.8\% 
    &
  29&
  12.1\%
\\ \hline
\multirow{2}{*}{Quad2} &
  Advancement &
  7 &
  4.3\% &
  1 &
  3.3\% &
  7 &
  4.3\% &
  1 &
  6.3\% &
  0 &
  0.0\% &
  2 &
  5.6\% &
  4 &
  2.9\% &
  2 &
  12.5\% 
    &
  8&
  4.1\%
  \\ \cline{2-20} 

 &
 
  Performance &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% 
    &
  0&
  0.0\%
  \\ \cline{2-20} 
 
 &
 
  Factual Contr. &
  62 &
  38.0\% &
  12 &
  40.0\% &
  61 &
  37.4\% &
  6 &
  37.5\% &
  1 &
  50.0\% &
  14 &
  38.9\% &
  52 &
  38.0\% &
  6 &
  37.5\% 
    &
  74&
  38.3\%
\\ \hline

\multirow{2}{*}{Quad3} &
  Self-Development &
  15 &
  9.2\% &
  4 &
  13.3\% &
  17 &
  10.3\% &
  1 &
  6.3\% &
  0 &
  0.0\% &
  2 &
  5.6\% &
  14 &
  10.2\% &
  2 &
  12.6\% 
  &
  19&
  9.8\%
  \\ \cline{2-20} 
 &
  Creativity &
  1 &
  0.6\% &
  1 &
  3.3\% &
  2 &
  1.2\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  1 &
  2.8\% &
  1 &
  0.7\% &
  0 &
  0.0\% 
    &
  2&
  0.9\%
\\ \hline

\multirow{2}{*}{Quad4} &
  Satisfaction &
  11 &
  6.7\% &
  3 &
  10.0\% &
  11 &
  6.6\% &
  1 &
  6.3\% &
  0 &
  0.0\% &
  1 &
  2.8\% &
  11 &
  8.0\% &
  1 &
  6.3\% 
  &
  13&
  5.4\%
  \\ \cline{2-20} 
 &
  Security &
  17 &
  10.4\% &
  0 &
  0.0\% &
  15 &
  9.0\% &
  2 &
  12.5\% &
  0 &
  0.0\% &
  3 &
  8.3\% &
  9 &
  6.6\% &
  5 &
  31.3\% 
  &
  17&
  7.1\%
  \\ \hline


\multicolumn{2}{r|}{Total unique resp.} &
  163 &
   &
  30 &
   &
  165 &
   &
  16 &
   &
  2 &
   &
  36 &
   &
  137 &
   &
  16 &
   & 193
  &
   \\ \hline
\end{tabular}
}

\resizebox{\textwidth}{!}{%
\tiny
\begin{tabular}{r}
\textbf{Quad1}: Interpersonal x Affect; \textbf{Quad2}: Interpersonal x Achievement; \textbf{Quad3}: Intrapersonal x Achievement; \textbf{Quad4}: Intrapersonal x Affect; \\
The sum of each quadrant can differ from the total of unique respondents as people often provided an answer to the open question that was categorized into more than one region. 
\end{tabular}
}

\end{table*}



==> Tables/mentors.tex <==
\begin{table}[htb]
\centering
\caption{Activities and behaviour of successful OSS mentors, according to our survey respondents}
\label{tab:mentors}

\resizebox{0.5\textwidth}{!}{%

\begin{tabular}{l|l}
\hline
\rowcolor[HTML]{C0C0C0} 
Being a successful mentor & \begin{tabular}[c]{@{}l@{}}Respondents’\\ IDs (Survey)\end{tabular} \\ \hline
\textit{''Delegate (instead of concentrate) work loads"} & S177     \\ \hline
\textit{''Motivate people"}                              & S6       \\ \hline
\textit{''Teach how to use the software"}                & S22      \\ \hline
\textit{''Help newcomers"}                               & S29, S37 \\ \hline
\textit{"Encourage and ground themselves in empathy"}    & S73      \\ \hline
\end{tabular}}
\end{table}

==> Tables/new_codes_survey.tex <==
\begin{table*}[htb]
\centering
\caption{How do survey respondents define a successful OSS contributor}
\label{tab:codes_survey_new}
\footnotesize
\resizebox{0.5\textwidth}{!}{%

\begin{tabular}{c|c|c|l|c|c}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Quadrant}                & \#                   & \%                       & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Region}} & \# & \%     \\ \hline\hline
                        &                      &                          & Cooperation                                         & 19 & 8.0\%  \\ \cline{4-6} 
                        &                      &                          & Perceived Contribution                              & 57 & 29.5\% \\ \cline{4-6} 
\multirow{-3}{*}{Quad1} & \multirow{-3}{*}{93} & \multirow{-3}{*}{48.2\%} & Recognition          & 29 & 12.1\% \\ \hline
                        &                      &                          & Advancement                                         & 8  & 4.1\%  \\ \cline{4-6} 
                        &                      &                          & Performance                                         & 0  & 0.0\%  \\ \cline{4-6} 
\multirow{-3}{*}{Quad2} & \multirow{-3}{*}{81} & \multirow{-3}{*}{42.0\%} & Factual Contribution & 74 & 38.3\% \\ \hline
                        &                      &                          & Self-Development                                    & 19 & 9.8\%  \\ \cline{4-6} 
\multirow{-2}{*}{Quad3} & \multirow{-2}{*}{21} & \multirow{-2}{*}{10.9\%} & Creativity                                          & 2  & 0.9\%  \\ \hline
                        &                      &                          & Satisfaction                                        & 13 & 5.4\%  \\ \cline{4-6} 
\multirow{-2}{*}{Quad4} & \multirow{-2}{*}{30} & \multirow{-2}{*}{15.5\%} & Security                                            & 17 & 7.1\%  \\ \hline\hline
\end{tabular}

}
\resizebox{0.80\textwidth}{!}{%
\tiny
\begin{tabular}{r}
\textbf{Quad1}: Interpersonal x Affect; \textbf{Quad2}: Interpersonal x Achievement; \textbf{Quad3}: Intrapersonal x Achievement; \textbf{Quad4}: Intrapersonal x Affect; \\
The sum of each quadrant can differ from the total of unique respondents as people often provided an answer to the open question that was categorized into more than one region. 
\end{tabular}
}
\end{table*}

==> Tables/recognition.tex <==
\begin{table}[htb]
\centering
\caption{Recognizing a successful OSS contributor, according to our survey respondents}
\label{tab:recognition}

\resizebox{0.5\textwidth}{!}{%

\begin{tabular}{l|l}
\hline
\rowcolor[HTML]{C0C0C0} 
Recognition Measures & \begin{tabular}[c]{@{}l@{}}Respondents’\\ IDs (Survey)\end{tabular} \\ \hline
\textit{''Have a high number of stars on the own} \\\textit{repository in Github"} & S58 and S109     \\ \hline
\textit{''Receive donations"} & S21       \\ \hline
\textit{''Be invited for conference invites/talks"} & S16 \\ \hline
\textit{''Have the name behind a relevant project,} \\\textit{library or application"} & S10 and S98 \\ \hline
\end{tabular}}
\end{table}

==> Tables/search_string.tex <==
\begin{table*}[htb]
\centering
\scriptsize
\caption{Database Search Strings, Filters and Results}
\label{tab:search_string}


\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Database} &
  \textbf{Search String} &
  Filters Applied &
  Results \\ \hline
Scopus &
  \begin{tabular}[c]{@{}c@{}}TITLE-ABS-KEY((woman OR women OR female OR gender OR  diversity OR "heterogeneous team") \\ AND ("open source" OR "open-source"  OR "free software" OR foss OR floss* OR oss))\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Included only\\  the ‘computer \\ science’ \\ category\end{tabular} &
  1067 \\ \hline
IEEE &
  \begin{tabular}[c]{@{}c@{}}("All Metadata":woman OR "All Metadata": women OR "All Metadata": diversity OR  \\ "All Metadata": female OR "All Metadata": "heterogeneous team" OR "All Metadata": gender) \\ AND ("All Metadata":"open source" OR "All Metadata":"open-source" \\ OR "All Metadata":"free software" OR "All Metadata": OSS \\ OR "All Metadata": FOSS OR "All Metadata": FLOSS*)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}No Filters \\ Were Used\end{tabular} &
  350 \\ \hline
Compendex &
  \begin{tabular}[c]{@{}c@{}}(((((woman OR women OR female OR gender OR  diversity  OR  "heterogeneous team") \\ AND ("open source"  OR  "open-source"  OR  "free software" OR foss OR  floss* OR oss))))\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}No Filters \\ Were Used\end{tabular} &
  100 \\ \hline
ACM &
  \begin{tabular}[c]{@{}c@{}}Title:(((woman OR women OR female OR gender OR diversity OR  "heterogeneous team") \\ AND ("open source" OR "open-source" OR "free software" OR foss OR floss* OR oss))) \\ OR Abstract:(((woman OR women OR gender OR diversity) \\ AND ("open source" OR "open-source" OR "free software" OR foss OR floss* OR oss))) \\ OR Keyword:(((woman OR women OR gender OR diversity) \\ AND ("open source" OR "open-source" OR "free software" OR foss OR floss* OR oss)))\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}No Filters \\ Were Used\end{tabular} &
  879 \\ \hline
\end{tabular}
\end{table*}

==> Tables/survey_demo.tex <==
\begin{table}[htb]
\centering
\caption{Demographics for the Survey Respondents}
\label{tab:survey_demo}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{c|c|ccc|c|c}
\cline{1-3}\cline{5-7}
\cellcolor{gray!35}\textbf{Role} & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}  & \multirow{15}{*}{} & \cellcolor{gray!35}\textbf{Country of Residence} & \cellcolor{gray!35}\textbf{\#} & \cellcolor{gray!35}\textbf{\%}\\\cline{1-3}\cline{5-7}
Coder              & 163 & 84.46\% &                    & Germany              & 89 & 46.11\% \\
Non-Coder          & 30  & 15.54\% &                    & USA                  & 59 & 30.57\% \\\cline{1-3}
\multicolumn{3}{l}{}               &                    & Netherlands          & 12 & 6.22\%  \\\cline{1-3}
\cellcolor{gray!35}\textbf{Gender}             & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}      &                    & Brazil               & 9  & 4.66\%  \\\cline{1-3}
Men                & 165 & 85.49\% &                    & Others               & 23 & 11.92\% \\
Women              & 16  & 8.29\%  &                    & Did not answer       & 1  & 0.52\%  \\\cline{5-7}
Non-Binary         & 2   & 1.04\%  &\multicolumn{1}{l}{}& \multicolumn{3}{l}{}                \\\cline{5-7}
Did not answer     & 10  & 5.18\%  &                    & \cellcolor{gray!35}\textbf{Age}  & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}      \\\cline{1-3}\cline{5-7}
\multicolumn{3}{l}{}               &                    & 24 or less           & 30 & 15.54\% \\\cline{1-3}
\cellcolor{gray!35}\textbf{Financial Relation} & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}       &                    & 25-34                & 60 & 31.09\% \\
Paid               & 36  & 18.65\% &                    & 35-44                & 59 & 30.57\% \\
Unpaid             & 137 & 70.98\% &                    & 45-54                & 27 & 13.99\% \\
Partially Paid     & 16  & 8.29\%  &                    & 55 or more           & 10 & 5.18\%  \\
Did not answer     & 4   & 2.07\%  &                    & Did not answer       & 7  & 3.63\% \\\cline{1-3}\cline{5-7}

\end{tabular}}
\end{table}

==> not_used.tex <==
The recommendations provided by our participants for \textsc{Self-Development}.

\review{\MyBox{
\textbf{\textsc{Develop technical skills and remember to...}}
\begin{itemize}
    \item Be pragmatic and try to learn as fast you can
    \item Read the project's documentation and understand both the architecture and how to create documentation
    \item Tinker with code if you are a code developer
    \item Join technical meetings and listen to the more experienced contributors
    \item Practice code reviews even when not being asked to
    \item Lurk since child and start early if you have the opportunity
\end{itemize}
}}

%\textsc{Technical:} 
Our participants suggested a new contributor to \textsc{be pragmatic and try to learn fast} (P19) through the following learning strategies: \textsc{reading the project's documentation} (P11,P18) to both absolve knowledge and learn how to document while making contributions, \textsc{tinkering with code} (P7) to learn code development by experimentation, and \textit{joining technical meetings} (P1,P20) to learn with more experienced contributors. Both P1 and P20 suggested being close (even remotely) to collaborate with peers to learn and grow. The proximity can happen in events as conferences and meetups and during regular contributions by asking and giving help to others. P6 mentioned he used to \textsc{practice code reviews} by \textit{``reviewing other people's code to improve [his] review skills, without being asked to do that, in addition to the contributions that [he] already had to make"}. The technical skills should be stimulated by \textsc{lurking since child} by \textit{``playing around and hacking stuff"} (P5), so the child discovers and is curious in programming. Moreover, the contributions should also \textsc{start early, since school} (P1).

%\textsc{Management:} 

\review{\MyBox{
\textbf{\textsc{Develop management skills and remember to...}}
\begin{itemize}
    \item Keep the tasks and processes unambiguous and well-documented
    \item Communicate with transparency
    \item Differentiate project and individual communication
    \item Negotiate to build consensus
\end{itemize}
Want to avoid burnout? Plan yourself to delegate tasks.
}}

When managing an OSS project, both P5 and P18 suggested to  \textsc{keep the tasks and processes unambiguous and well-documented}. According to P1, P3, and P4, you need to document to be able to \textsc{delegate tasks} to other contributors, so you do not concentrate the work on yourself, and people can help you or work in your absence. In terms of communication, P16 suggested to \textsc{differentiate project and individual communication} to \textsc{provide transparency} on all layers of the process as possible. So, \textit{``if you have something to say to someone, individually, you contact them over email, but for project related decisions, we use a lot of mailing lists, or forums, all of the discussion is public"} (P16). Even when discussing something related to the project in person, \textsc{negotiate to build consensus} (P6) and make sure to document to provide transparency, ``otherwise, you're just creating a closed community" (P5).

\review{\MyBox{
\textbf{\textsc{Adapt you personality and remember to...}}
\begin{itemize}
    \item Be open minded and confident to accept critiques and not to take them personally
    \item Have diligence to keep a frequency the of study and learn
    \item Have a positive attitude and bring solutions, not only problems
    \item Do not accommodate in the same position
    \item Have role models and watch how they do work
\end{itemize}
Do not know how to start? Inspire yourself by choosing a project you are passionate in.}}

%\textsc{Personality:} 
Learning is an ongoing process, and our participants considered that a contributor should \textsc{have diligence to \textit{``keep a frequency the of study and learn"}} (P21). When making contributions and receiving comments, P2 advised to be \textsc{open minded to accept critiques to your work} and \textit{``understand that critiques are for the code and not for you"}. According to P15 and P16, you need to have \textsc{confidence not to take the critiques personally} \textit{``as an attack"}. P8 complemented suggesting for when receiving a comment, \textit{`` learn to do better or differently [...] and iterate and iterate and iterate"} as doing a retrospective of own actions to improve next time. When giving the first steps, \textit{``be ready to try and commit mistakes"} (P2) and remember to \textsc{have a positive attitude and bring solutions}, instead of only exposing problems (P7). P19 advised to  \textit{``\textsc{not accommodate in the same position}, try to advance in the project hierarchy as soon you can"} to progress and grow in the OSS career. One suggestion to achieve some improvement of own work is to \textsc{have role models and ``watch how they do work}, what and how are they doing, what are the skills that they need, and just trying to pick up some of those things and be better, in general" (P4). Newcomers should find their way to start from scratch (P9) by \textsc{choosing a project \textit{``[they] are passionate in}} (P1), studying the rules of that community before starting (P2,P8) and find something to help and add value, even not technically (P1,P9).

\review{\MyBox{
\textbf{\textsc{Develop social skills and remember to...}}
\begin{itemize}
    \item Learn English
    \item Develop both writing and verbal communication skills
    \item Employ empathy during interactions
    \item Influence and argument using benefits and rewards
    \item Help others to grow
    \item Use flexibility to interact with different cultures
\end{itemize}
OSS is all about people and community. Bond to the community, specially if you are going to speak for it.
}}

\textsc{Social:}
Although OSS comprises a diverse set of contributors and people who collaborate are spread around the globe, speaking many different languages, both P5 and P20 agreed that \textsc{learning English} can help to reduce entry barriers, as most of everything is still in English. According to our participants, \textsc{developing written and verbal communication skills} are essential for success for all contributors in OSS (P6, P7, P8, P11, P19), as exposed by P6: \textit{``Technical writing, and speaking, and general communication is critical. [..] Being able to talk about it and describe it both written word eloquently and verbally is absolutely cool"}. First step to develop communication skills is becoming a good listener (P8), \textit{``ask good questions and listen"} (P11). Another aspect of learning about communication is that \textit{``everyone communicates differently, so you need to understand that"} (P4) to communicate with people using different tools. In a broader spectrum, P3 and P15 mentioned that is important to develop and yourself in \textsc{flexibility to interact with different cultures}. The interactions between people from different cultures in OSS happen all the time, as OSS contributors who collaborate in the projects are usually spread around the globe. Abruptly interrupting a meeting that reached the scheduled time, for example, can be commonplace for people from American culture but represent an insult for people from Middle Eastern culture (P15). Indeed, learning how to interact and building relationships are fundamental skills for OSS contributors, \textit{``because OSS is people, it is not GitHub, it is not repositories, it is not cold, it is not software"} (P10). The excellent communication style should arrive from the core members of the community, \textit{``come from a herd mentality"} (P6). According to P22, a contributor needs to \textsc{employ empathy during interactions} and ``be good with people". Empathy is a concept that can avoid many communication hurdles when one ``tries to understand another person's perspective [..] and asks yourself why would someone make that choice" (P8). Before sending an email or chat message, \textit{``remember that at the other end is a person who may be having a crappy day"} (P15). P3 suggested to  \textsc{be a leader who helps others to grow} and being a \textit{``servant leader [...] pulling up people behind"} (P3). P15 complement with the abilities to \textsc{influence and argument using benefits and rewards}, instead of only giving orders. Our participants highlighted the need to \textsc{bond to the community}, \textit{``be true"} (P17) to it, and commit to the OSS philosophy. As stated by P10: \textit{``build a relationship with a community is crucial, especially if you are willing to speak for it"}.
%In a traditional workplace, the social atmosphere is one of the aspects of well-being that can impact employees' productivity and retention \cite{clements2006creating, warr1998our}. When recruiting new employees, many companies look at the technical skills and whether a potential employee fits well within the company culture and vision. In OSS, the social environment is even more critical. In this category, we grouped the pieces of advice provided by our participants to develop skills that help contributors to deal with other contributors, who might not have the same culture, maybe not speak the same language, or not know how to get started \cite{dias2021makes}.
%Contributing to OSS can be challenging as contributors have to understand the codebase and its architecture, but also the behavior rules, tools, and technology employed and required by each project ~\cite{steinmacher2015social, balali2020recommending, padala2020gender}. The lack of technical background and domain expertise can hinder the contribution process~\cite{steinmacher2018almost,steinmacher2015social}.
%Peripheral developers can represent very active promoters of the products with which they are involved, enhancing product awareness and being word-of-mouth agents through their personal channels (such as their blogs and websites) \cite{setia2012peripheral}. 

%%%% RECOMMENDATION FOR PRACTITIONERS %%%%%

\review{\section{Recommendations for Practitioners and Implications for Communities and Researchers}
\label{sec:recommendations}}

In addition to the implications mentioned as part of the discussion, we highlight \review{recommendations provided by our participants for practitioners}, and another set of ways that our results may inspire researchers and communities. 

\review{\subsection{Recommendation for Practitioners}}

\review{We organized the recommendation for practitioners to be successful from both our participants and literature using the four quadrants of the multidimensional  model of success proposed by Dries et al.~\cite{dries2008career} (see Section~\ref{sec:background}). 

\MyBox{
\textbf{Recommendations to support achieving OSS success in Quad1 (Cooperation, Perceived Contribution, and Recognition)}
\begin{itemize}
    \item Participate on different meetups
    \item Bring who is not participating
    \item Contribute to important technical issues
    \item Answer questions and discuss features
    \item Create impactful technology or messages
    \item Create a portfolio of contributions
\end{itemize}
}

%\textbf{\textsc{Cooperation}} for our participants involved expanding own networking, supporting the community growth and mentoring newcomers. 
Attending events and meetups is a straightforward way to increase personal networks and \textbf{\textsc{Cooperation}}  \cite{borges2019developers,ingram2020software}. During our interviews, it was mentioned as a key to success for P1, P13, and P20. P1 and P20 suggested that events can be useful to stay close (even remotely) to  peers and have a chance to ask for help and to meet people during informal conversations.
%P8 advised mentees to not \textit{``put so much weight on the shoulders of mentorship"} because usually, the mentors are overloaded. The recommendation for mentors was about managing time in mentorship. In addition to the traditional dyadic form of mentoring, OSS mentors also take part in a network-enabled form of collective feedback~\cite{campbell2016thousands}. P1 recommended this strategy to save time by doing \textit{``scalable mentoring sessions [...], as being on Slack channel on a daily basis to take questions for 20 minutes"}. 
%On the other side, P8 advised mentees to not \textit{``put so much weight on the shoulders of mentorship"} because usually, the mentors are overloaded. Instead, proactively ask for help during an informal conversation.

\textbf{\textsc{Perceived Contribution}} includes how others see one's personal success associated to the project's success or outreach. To do so, during the interviews, P6 recommended to ``treat [the software] as a business [..] trying to get people to use the software.'' Complementing that, P11 reminded that it is important to \textit{look at who is not participating, who we are not reaching, because there's a reason we're not reaching them, whatever that reason might be, we haven't done outreach in a foreign country, or whatever it is.} Therefore, it is important to use marketing strategies, for example, by creating informative and persuasive communication to increase the diffusion outcomes of a product (awareness and adoption)~\cite{kalish1985new}. By having a popular project, it is possible to increase the perceived contribution of the team behind the project.

In order to gain \textbf{\textsc{Recognition}}, the contributors have to start with small steps by behaving humbly and contributing code related to important technical issues. Even for non-coders, the contributor should build their reputation by demonstrating expertise and increase their credibility. For example, one can build their name by answering  questions and discussing issues and feature requests, and may ultimately evolve to a trustful source and somewhat of a philosopher~\cite{ducheneaut2005socialization}. As suggested by P27, you should have people following you by \textit{"creating impactful technology, or stating impactful messages [...], so you have visibility and `when people read your name, they know what you have done.'''} For example, code contributors can use their history of contributions as a portfolio, so they can be referred by potential employers~\cite{7111876}---\textit{"make public contributions, GitHub is a network of job opportunities"} (P19).
. %P1 suggested: \textit{"if you are a coder, gain credibility as a coder"} and P19 complemented: 

\MyBox{
\textbf{Recommendations to support achieving OSS success in Quad2 (Factual Contribution, Performance and Advancement)}
\begin{itemize}
    \item Study the community rules before starting
    \item Find something to help and add value 
    \item Have a positive attitude and bring solutions
    \item Do not accommodate in the same position
\end{itemize}
}

Regarding Quad 2, according to our participants, contributors should find their way to start from scratch (P9) to bring \textbf{\textsc{Factual Contributions}} by reading documentation and studying the rules of that community before starting (P2,P8), finding something to help and add value, even not technically (P1,P9). When giving the first steps, \textit{``be ready to try and commit mistakes"} (P2) and remember to have a positive attitude and bring solutions, instead of only exposing problems (P7). 
%One strategy to sell services is offer consultancy and specialized support of an OSS \cite{fitzgerald2006transformation}.
P19 also recommended proactive attitude in case you want to focus on \textbf{\textsc{Advancement}}: \textit{``[do] not accommodate in the same position, try to advance in the project hierarchy as soon you can"} to progress and grow in the OSS career. Merit-based rankings communicates important information to contributors about their \textbf{\textsc{Performance}}, ability and productive capacity in software development as well as the value of their contributions to the OSS community \cite{roberts2006understanding}.

\MyBox{
\textbf{Recommendations to support achieving OSS success in Quad3 (Self-Development and Creativity)}
\begin{itemize}
    \item Have diligence to keep a frequency the of study
    \item Tinker with code to learn from experimentation
    \item Join technical meetings to learn from listening more experienced contributors
    \item Practice code reviews to learn from practice
    \item Be open minded to learn from feedback
    \item Be a good listener to acquire communication skills
    \item Be flexible when interacting with diverse cultures
\end{itemize}
}
When success is related to \textsc{\textbf{Self-Development}}, %, and besides summer of code programs, that connect students to OSS projects, typically during the summer break from school~\cite{SILVA2020110487}, 
our participants recommend that a contributor should be diligent to \textit{``keep a frequency the of study and learn"} (P21). Tinkering with code (P7) to learn code development by experimentation, joining technical meetings (P1,P20) to learn with more experienced contributors, and practicing code reviews by \textit{``reviewing other people's code to improve [their] review skills"} (P6) also helps in this aspect. When making contributions and receiving comments, P2 recommended to be open minded to learn from feedback by \textit{``understanding that critiques are for the code and not for you"}. Developing relational skills is also important. According to our respondents, social cultural relationship (P3,P15), English for both verbal and written interactions, and empathy (P22) are crucial \textit{``because OSS is people, it is not GitHub, it is not repositories, it is not cold, it is not software"} (P10).
Developing yourself in flexibility is important to learn how to interact with different cultures (P3,P15), as OSS contributors who collaborate in the projects are usually spread around the globe. Abruptly interrupting a meeting that reached the scheduled time, for example, can be commonplace for people from American culture but represent an insult for people from Middle Eastern culture (P15). %Indeed, learning how to interact and building relationships are fundamental skills for OSS contributors, \textit{``because OSS is people, it is not GitHub, it is not repositories, it is not cold, it is not software"} (P10). The excellent communication style should arrive from the core members of the community, \textit{``come from a herd mentality"} (P6). 
%According to P22, a contributor needs to have empathy during interactions and ``be good with people" to develop communication skills . Empathy is a concept that can avoid many communication hurdles when one ``tries to understand another person's perspective [..] and asks yourself why would someone make that choice" (P8). Before sending an email or chat message, \textit{``remember that at the other end is a person who may be having a crappy day"} (P15).
%P15 also mentioned the need to developing management abilities to negotiate and influence and argument using benefits and rewards, instead of only giving orders.

\MyBox{
\textbf{Recommendations to support achieving OSS success in Quad4 (Security and Satisfaction)}
\begin{itemize}
    \item Choose a project you are passionate in
    \item Learn how to delegate tasks and avoid burnout
    \item Apply for a job in OSS
\end{itemize}
}

In order to \textit{``derive \textsc{Satisfaction} from work"} (P12), a contributor should \textit{find a project ``[they] are passionate in [..] and have a job [they] want to wake up for every day} (P1).  However, P1 and P6 warned to be careful and avoid burnout, which can affect well-being and happiness \cite{graziotin2018happens,nowogrodzki2019support}. Project key members often report high stress levels from frequent demands for features and bug fixes and from the sometimes aggressive tone of these demands \cite{raman2020stress}. Delegating tasks is one strategy mentioned by our participants to avoid burnout so contributors do not concentrate the work in themselves (P1,P3,P4). In order to delegate tasks to other contributors, P1, P5 and P18 recommended to keep the tasks and processes unambiguous and well-documented. 

About half of all code contributions are being performed during regular work times, from Monday to Friday between 9 am and 5PM, likewise suggesting that many OSS contributors are having the \textsc{Security} to make a living from OSS \cite{riehle2015open}. High-profile organizations like Amazon, Google, and Salesforce use OSS behind their products and have jobs in OSS \cite{fitzgerald2006transformation} and are interested in having core reviewers among their staff \cite{van2017reviewing}. However, a contributor can have different backgrounds and follow different pathways in OSS, even not being a software developer \cite{trinkenreich2020pathways}. Most of our interviewees work for big companies and foundations, including the Linux Foundation, Microsoft, Google, IBM, Bitergia, Red Hat, and GitLab. Another option to earn some dollars from contributing is
by bounties that are payments per solved issues. However, the value of each bounty is usually low and only a few hunters earn more than \$2,000 \cite{zhou2021studying}.}
